Efficient Bound of Lipschitz Constant for Convolutional Layers by Gram Iteration

Since the control of the Lipschitz constant has a great impact on the training stability, generalization, and robustness of neural networks, the estimation of this value is nowadays a real scientific challenge. In this paper we introduce a precise, fast, and differentiable upper bound for the spectral norm of convolutional layers using circulant matrix theory and a new alternative to the Power iteration. Called the Gram iteration, our approach exhibits a superlinear convergence. First, we show through a comprehensive set of experiments that our approach outperforms other state-of-the-art methods in terms of precision, computational cost, and scalability. Then, it proves highly effective for the Lipschitz regularization of convolutional neural networks, with competitive results against concurrent approaches. Code is available at https://github.com/blaisedelattre/lip4conv.

==> sections/archive.tex <==
\subsection{Doubly block circulant matrix}
\blaise{Ecrire avec multi level circulant matrix, puis se faire un dessin}
For a row $a =(a_1, a_2, a_3)$ the associated circulant matrix is:
\begin{equation*}
A = \text{circ}(a) = 
\begin{pmatrix}
a_{0} & a_{1} & a_{2} \\
a_{2} & a_{0} & a_{1} \\
a_{1} & a_{2} & a_{0} \\ 
\end{pmatrix}
\end{equation*}

Circulant matrix can represent circular convolution, 
for a vector $x$, $Ax = b$ can be write as the equation of circular convolution: $a \ast x = b$.

The discrete Fourier transform matrix diagonalizes A:
$U^* = \frac{1}{\sqrt{n} }F$ and $U = \frac{1}{\sqrt{n} }F^{-1} \in \mathbb{C}^{n \times n }$.
%$$A = U^* \diag(F a) U$$
$$A = U^* \diag(\tilde{a}) U \ ,$$ where $\Tilde{a} = F a \in \mathbb{C}^{n}$ is the Fourier transform of $a$.

In the case where input channels and output channels are one : $\cout=\cin=1$. For an input $x \in \mathbb{R}^{n \times n}$.
Consider two dimension kernel ${k \times k}$ matrix that we embed in a $n \times n$ matrix by padding with zeros, $K \in \mathbb{R}^{n \times n}$. \\
A doubly-block circulant matrix is a block matrix where each block is itself a circulant matrix. \\

\begin{align*}
A &= \text{circ}(K) \\ &=
\begin{pmatrix}
\text{circ}(K_{1}) & \text{circ}(K_{2}) & \dots & \text{circ}(K_{n}) \\
\text{circ}(K_{n}) & \text{circ}(K_{1}) & \dots & \text{circ}(K_{n-1}) \\
\vdots & \vdots & \ddots & \vdots \\
\text{circ}(K_{2}) & \text{circ}(K_{3}) & \dots & \text{circ}(K_{1}) \\
\end{pmatrix}
\end{align*}

The linear transformation for the convolution $K \ast x = y$
can be represent with the  matrix vecotr product 
$A \vect{x} = \vect{y}$.
Similarly the 2D Fourier transform diagonalizes $A$.
$A = U^* \diag(\vect{\Tilde{K}}) U$ with
$U^* = \frac{1}{n} F \otimes F $ and $U = \frac{1}{n} F^{-1} \otimes F^{-1} \in \mathbb{R}^{n^2 \times n^2}$.

When $\cin, \cout \geq 1$, $K \in \mathbb{R}^{\cout \times \cin \times n \times n}$
\begin{equation*}
A = 
\begin{pmatrix}
\text{circ}(K_{1, 1})  
%& \text{circ}(K[1, 2]) 
& \dots & \text{circ}(K_{1, \cin}) \\
\text{circ}(K_{2, 1}) 
%& \text{circ}(K[2, 2]) 
& \dots & \text{circ}(K_{2, \cin}) \\
%\vdots & 
\vdots & \ddots & \vdots \\
\text{circ}(K_{\cout,1}) 
%& \text{circ}(K[\cout,2]) 
& \dots & \text{circ}(K_{\cout,\cin}) \\
\end{pmatrix}
\end{equation*}

Let us call $D_{i,j} = \diag( \vect{ \Tilde{K}_{i, j}})$ the element $i,j$ of block matrix $D$:

\begin{equation*}
D = 
\begin{pmatrix}
D_{1,1} & \dots &  D_{1,\cin}  \\
\vdots & \ddots & \vdots \\
D_{\cout,1} & \dots & D_{\cout,\cin} \\
\end{pmatrix}
\end{equation*}

Then, \begin{align*}
A &= 
\begin{pmatrix}
U^\dag D_{1,1} U & \dots & U^\dag D_{1,\cin} U \\
\vdots & \ddots & \vdots \\
U^\dag D_{\cout,1} U & \dots & U^\dag D_{\cout,\cin} U \\
\end{pmatrix}
\\
&= R
\begin{pmatrix}
D_{1,1} & \dots & D_{1,\cin} \\
\vdots & \ddots & \vdots \\
 D_{\cout,1} & \dots & D_{\cout,\cin} \\
\end{pmatrix}
Q
\end{align*}

with $R = I_\cin \otimes U^\dag \in \mathbb{R}^{\cin n^2 \times \cin n^2}$,
$Q = I_\cout \otimes U \in \mathbb{R}^{\cout n^2 \times \cout n^2}$,
note that $R$ and $Q$ are normal.
$R^{\dag} R = (I_\cin \otimes U)(I_\cin \otimes U^{\dag}) = (I_\cin I_\cin)\otimes (U U^{\dag}) = I_{\cin n^2}$.
Likewise $Q^{\dag} Q = I_{\cout n^2}$.
Hence singular values of $A=RDQ$ are the same as $D$. \\


\section{Theoritical Framework}

\blaise{Figure style OCNN}
Introduce  $G_{u,v, i, j} = D_{i,j,u,v}$. $G_{u,v}$ is a $c_{out} \times c_{in}$ matrix. From \cite{sedghi2018singular}, the singular values $\sigma$ of 
\begin{equation*}
A =
R
\begin{pmatrix}
D_{1,1} & \dots &  D_{1,\cin}  \\
\vdots & \ddots & \vdots \\
 D_{\cout,1} & \dots & D_{\cout,\cin}  \\
\end{pmatrix}
Q
\end{equation*}

are given by :
\begin{align}
\label{eq:bounds_singular_values}
\sigma(A) = \bigcup_{1 \leq u,v \leq n} \sigma({G_{u,v}})   
\end{align}
%\blaise{Bon, si jamais on note : \begin{align}\sigma(A) = \bigcup_{1 \leq u,v \leq n} \sigma({D_{:,:,u,v}})   \end{align}est ce que c'est plus ou moins clair ?Si oui pas besoin des $G$ défini plus haut}
We have $G_{u,v} = [[F^\top K_{i, j} F]_{u,v}]_{i,j}$,
with $1 \leq i \leq \cout$ and $1 \leq j \leq \cin$.

\begin{prop}
%$$\sigma_1(A) \leq \sqrt{ \max_{1 \leq u,v \leq n} \sum_{i=1}^\cout \sum_{j=1}^\cin \left| \vect{\Tilde{K}_{i,j}} \right|^2_{u,v}}$$
$$\sigma_1(A) \leq \max_{1 \leq u,v \leq n} \norm{G_{u,v}}_F$$
\end{prop}

\begin{proof}
Equation \ref{eq:bounds_singular_values} gives a bound on the maximum singular values of $A$ : 

$\sigma_1(A) = \max_{1 \leq i,j \leq n} \sigma_1({G_{u,v}})  $

Using that $\sigma_1({G_{u,v}}) \leq \norm{G_{u,v}}_F$ we have the result.
\end{proof}
Finally expressing with $K$ :
\begin{prop}
$$\sigma_1(A) \leq \max_{1 \leq u,v \leq n} 
%\left[ 
\sum_{\substack{1 \leq i \leq \cout \\ 1 \leq j \leq \cin}}  \Tilde{K}_{i, j,u,v} %\right]_{u,v}
$$
\end{prop}

\subsection{Generalisation}
For $G \in \{ G_{u,v} : 1 \leq u,v \leq n \}$,
consider 
 $G = V \Gamma W^\dag$ the singular values decomposition of $G$. With $\Gamma = \diag(\gamma)$, $\gamma = (\gamma_1, \dots, \gamma_m)$ and $m = \min(\cin, \cout)$. We use the convention $|\gamma_1| \geq |\gamma_2| \geq \dots \geq |\gamma_m|$

Define $G^t$, $\forall t \geq 1$:
\begin{align*}
   \left\{
    \begin{array}{ll}
    G^1 &= G^\dag G \\
    G^{t+1} &= {G^t}^\dag G^t
    \end{array} 
    \right.
\end{align*}

We get $G^{t} = W |\Gamma|^{2t} W^\dag, \forall t \geq 1$

\begin{prop}
\label{bound:max_frob_gt}
$$
\sigma_1(A) \leq \max_{1 \leq u,v \leq n} \sqrt[2t]{  \norm{G_{u,v}^t}_F}$$
\end{prop}

\begin{proof}

\begin{align*}
    \sigma_1(G_{u,v}) &=\sqrt[2t]{\sigma_1(G_{u,v}^t)} \\
    \sigma_1(G_{u,v}) &\leq \sqrt[2t]{
    \norm{
    {G^t_{u,v}}}_F
    }
\end{align*}

Then,
\begin{align*}
    \sigma_1(A) &\leq \max_{1 \leq u,v \leq n} \sigma_1(G_{u,v}) \\
    \sigma_1(A) &\leq \max_{1 \leq u,v \leq n} \sqrt[2t]{\norm{G_{u,v}^t}_F} \\
\end{align*}
\end{proof}



\begin{prop}
\label{bound:frob_gt_convergence}
For $G \in \{ G_{u,v} : 1 \leq u,v \leq n \}$,

$$
\sqrt[2t]{\norm{G^t}_F} \underset{t \to +\infty}{\longrightarrow} \sigma_1(G)
$$
\end{prop}

\begin{proof}

\begin{align*}
 \norm{G^t}_F^2 &= \text{Tr}(W |\Gamma|^{2t} W^\dag W |\Gamma|^{2t} W^\dag)\\
 \norm{G^t}_F^2 &= \text{Tr}(W |\Gamma|^{4t} W^\dag)\\
 \norm{G^t}_F^2 &= \text{Tr}(W^\dag W |\Gamma|^{4t} )\\
 \norm{G^t}_F^2 &= \text{Tr}(|\Gamma|^{4t}) \\
 \norm{G^t}_F^2 &= \sum_{i=1}^m |\gamma_i|^{4t}
\end{align*}
\begin{align*}
    \sqrt[4t]{||G^t||_F^2} &= \sqrt[4t]{\sum_{i=1}^m |\gamma_i|^{4t}}\\
    \sqrt[2t]{||G^t||_F} &= \sqrt[4t]{\sum_{i=1}^m |\gamma_i|^{4t}}\\
    \sqrt[2t]{||G^t||_F} &= \norm{\gamma}_{4t} \underset{t \to +\infty}{\longrightarrow} \norm{\gamma}_\infty\\
\end{align*}


and $\norm{\gamma}_\infty = \max_{1 \leq l \leq m}|\gamma|_l = \sigma_1(G)$
\end{proof}

Finally, using proposition \ref{bound:max_frob_gt} and \ref{bound:frob_gt_convergence} we have 

\begin{prop}
\label{bound:version_two}
$$
\sigma_1(A) \leq \max_{1 \leq u,v \leq n} \sqrt[2t]{  \norm{G^t_{u,v}}_F} \underset{t\to +\infty}{\longrightarrow} \sigma_1(A)
$$
\end{prop}

\blaise{En annexe ? preuve en annexe en tout cas}
\begin{prop}
\label{prop:convergence_rate}
The convergence is linear 
with rate $\left| \frac{\gamma_2}{\gamma_1} \right |$ (same as power iteration method).
\end{prop}

\begin{proof}
\label{proof:convergence_rate}
For $t \geq 1$, 
\begin{align*}
    \norm{\gamma}_{t} - \norm{\gamma}_{\infty} &= \norm{\gamma}_{\infty}
   \left(
   \frac{\norm{\gamma}_{t}}{\norm{\gamma}_{\infty}} - 1
   \right)\\
   &= \norm{\gamma}_{\infty}
   \left(
         \left(\sum_i 
                \frac{|\gamma_i|^t}
                {\norm{\gamma}_{\infty}^t}
          \right)^{1/t}
         - 1
   \right)\\
   &= \norm{\gamma}_{\infty}
   \left(
         \exp{ \left( \frac{1}{t}
                \log{\sum_i 
                \frac{|\gamma_i|^t}
                {\norm{\gamma}_{\infty}^t}}
          \right)}
         - 1
   \right)\\
   \end{align*}
   
\begin{align*}
   \log{\sum_i \frac{|\gamma_i|^t}{\norm{\gamma}_{\infty}^t}} &= 
    \log{ \left( 1 + \alpha \right)}\\
    \alpha &= 
    \sum_{i \neq i_{\text{max}}} 
    \frac{|\gamma_i|^t}
    {\norm{\gamma}_{\infty}^t} \underset{t\to +\infty}{\longrightarrow} 0\\
    \log{\sum_i \frac{|\gamma_i|^t}{\norm{\gamma}_{\infty}^t}} &\underset{t \to +\infty}{=} \alpha + o(\alpha^2)
\end{align*}

\begin{align*}
\norm{\gamma}_{t} - \norm{\gamma}_{\infty} &\underset{t \to +\infty}{=} \norm{\gamma}_{\infty}
   \left(
         (1 + \frac{1}{t} \alpha + o(\alpha^2)) -1
   \right)\\
   &\underset{t \to +\infty}{=} \frac{\norm{\gamma}_{\infty}}{t}
   \left(
         \alpha + o(\alpha^2)
   \right)\\
\end{align*}
 
 Hence 
 
 \begin{align*}
 \frac{\norm{\gamma}_{t+1} - \norm{\gamma}_{\infty}}
 {\norm{\gamma}_{t} - \norm{\gamma}_{\infty}} &
 \underset{t \to +\infty}{\sim}
 \frac{t}{t+1}
 \frac{\sum_{i \neq i_{\text{max}}} 
        \frac{|\gamma_i|^{t+1}}
        {\norm{\gamma}_{\infty}^{t+1}}
      }
      {\sum_{i \neq i_{\text{max}}} 
        \frac{|\gamma_i|^t}
        {\norm{\gamma}_{\infty}^t}
      }\\
\frac{\norm{\gamma}_{t+1} - \norm{\gamma}_{\infty}}
     {\norm{\gamma}_{t} - \norm{\gamma}_{\infty}} &
     \underset{t \to +\infty}{\sim}
     \frac{1}{\norm{\gamma}_{\infty}}
     \frac{\sum_{i \neq i_{\text{max}}} 
            |\gamma_i| |\gamma_i|^{t}
          }
          {\sum_{i \neq i_{\text{max}}} 
            |\gamma_i|^t
          }\\
     \frac{1}{\norm{\gamma}_{\infty}}
     \frac{\sum_{i \neq i_{\text{max}}} 
            |\gamma_i||\gamma_i|^{t}
          }
          {\sum_{i \neq i_{\text{max}}} 
            |\gamma_i|^t
          } &\leq 
          \frac{|\gamma_2|}{\norm{\gamma}_{\infty}} =
          \left|\frac{\gamma_2}{\gamma_1}\right|
     \\
 \end{align*}
\end{proof}




\section{Lipschitz bound of CNN}

\quentin{calcul des Lipschitz des autres couches! Trouver des refs!}

linear/dense layers

non-linear scalar operators, non-expansive: ReLu, sigmoid, etc

max-pooling

Estimation for batch normalization is given in Appendix C.4.1 of \cite{tsuzuku2018lipschitz}:
$$\max_i \{ \left| \gamma_i \right| / \sqrt{\sigma_i^2 + \epsilon} \}$$
This Lipschitz constant is rarely considered in the global constant of NNs.

residual connections and bottleneck blocks for ResNets




\section{Cheaper approximation}
This method requires to compute the $fft2$ for an $n \times n$ kernel several times. It can be expensive we large image size.

Let us define the primitive $n$-th root of unity $w_n = e^{-2\pi i /n}$, in which $i^2 = -1$. 

Starting from the expression
\begin{align}
||A_p||_2^2 &= \max_{i \leq n^2} \sum_{j=1}^{c} \left|\vect{\tilde{K}[p, j]}\right|^2_i \\
&= \max_{q,l, \leq n} \sum_{j=1}^{c} \left|\sum_{k_1=1}^{n} \sum_{k_2=1}^{n} w_n^{lk_1} w_n^{qk_2} K[p, j,k_1,k_2)]\right|^2 \\
&= \max_{q,l, \leq n} \sum_{j=1}^{c} \left|\sum_{k_1=1}^{k} \sum_{k_2=1}^{k} w_n^{lk_1 + qk_2}  K[p, j,k_1,k_2]\right|^2 \\
&= \max_{q,l, \leq n} \sum_{j=1}^{c} \left|\sum_{k_1=1}^{k} \sum_{k_2=1}^{k} e^{-2\pi i\frac{lk_1 + qk_2}{n}} K[p, j,k_1,k_2]\right|^2 \\
&= \max_{q,l, \leq n} \sum_{j=1}^{c} \left|\sum_{k_1=1}^{k} \sum_{k_2=1}^{k} e^{-i2\pi\frac{l}{n}k_1 + -i2\pi\frac{q}{n}k_1} K[p, j,k_1,k_2]\right|^2 \\
&= \max_{w_1,w_2, \in \{2\pi l/n ~ | ~ l \in [1,\dots, n] \}} \sum_{j=1}^{c} \left|\sum_{k_1=1}^{k} \sum_{k_2=1}^{k} e^{i (w_1 k_1 + w_2 k_1)} K[p, j,k_1,k_2]\right|^2 \\
&= \max_{w_1,w_2, \in \{2\pi l/n ~ | ~ l \in [1,\dots, n] \}} \sum_{j=1}^{c} \left|f_{pj} (w_1, w_2)\right|^2 \\
&\leq \max_{w_1,w_1, \in [0, 2\pi]} \sum_{j=1}^{c} \left|f_{pj} (w_1, w_2)\right|^2
\end{align}
The term $n$ appears as the parameter of equidistant sampling in a PolyGrid search to approximate (5) with (4). We can also pick $n_0 \leq n$ which accounts for a smaller number of sampling. \\
We can embed the $k \times k$ kernel matrix in a smaller $n_0 \times n_0$ to make the method cheaper. Work of Pfister and Bresler (2018) which analyzed the quality of approximation depending on $n_0$. \\

Taking 
$k \leq n_0 \leq n$. \\
We have 

$\max_{w_1,w_1, \in [0, 2\pi]} \sum_{j=1}^{c} |f_{pj}(w_1, w_2)|^2$


$\leq \frac{1}{1 - \alpha} \max_{w_1,w_2, \in \{2\pi l/n ~ | ~ l \in [1,\dots, n] \}} \sum_{j=1}^{c} |f_{pj} (w_1, w_2)|^2 \\
$

with $\alpha = \frac{2 \lfloor k /2 \rfloor}{n_0^2}$

Finally,

\begin{prop}
$$||A||_2 \leq \frac{1}{1 - \alpha} \sqrt{\sum_{p=1}^f \max_{i \leq n^2} \sum_{j=1}^{c} \left|\vect{\Tilde{K}_{n_0}[p,j]} \right|^2_i}$$
with $\alpha = \frac{2 \lfloor k /2 \rfloor}{n_0^2}$
\end{prop}



\section{To remove later : First Bound}
\label{section:global_framework}


In the case where there is one output channel $1 \leq p \leq \cout$ and $\cin \geq 1$.
$A_p = (D_{p,1}, D_{p,2}, \dots, D_{p,\cin})$ 

\begin{prop}

$$\sigma_1(A[p]) = \sqrt{\max_{i \leq n^2} \sum_{j=1}^{\cin} \left| \vect{\Tilde{K}[p, j]} \right|^2_i}$$

\end{prop}

\begin{proof}
\begin{align*}
\sigma_1(A[p])^2 &= \lambda_1(A[p] A^\dag[p])  \\
&= \lambda_1(\sum_{j=1}^{\cin}D[p,j] D^\dag[p,j])\\
&= \lambda_1(\sum_{j=1}^{\cin} \left|D[p,j]\right|^2 )\\
&= \max_{i \leq n^2} \sum_{j=1}^{\cin} \left|D[p,j]\right|^2_i \\
&= \max_{i \leq n^2} \sum_{j=1}^{\cin} \left| \vect{ \Tilde{K}[p, j]} \right|^2_i
\end{align*}
\end{proof}

In the case where $\cout, \cin \geq 1$

\begin{lemma}
\label{lemma:concat_singular_value}
For
$M = (M_1^\top, M_2^\top, \dots, M_m^\top)^\top$.
We can bound the spectral norm of $M$ as follows : 
$$\sigma_1(M) \leq \sqrt{\sum_{i=1}^m \sigma_1(M_i)^2}$$
\end{lemma}


Finally,

\begin{prop}
$$\sigma_1(A) \leq \sqrt{\sum_{p=1}^\cout \max_{i \leq n^2} \sum_{j=1}^{\cin} \left| \vect{\Tilde{K}[p,j]} \right|^2_i}$$

\end{prop}

\section{To remove later : Third Bound}
$A \in \mathbb{R}^{\cout n^2 \times \cin n^2}$

\begin{equation*}
A = 
\begin{pmatrix}
D[1,1] & \dots &  D[1,c] &  \\
\vdots & \ddots & \vdots \\
 D[f,1] &  \dots & D[f,c] &  \\
\end{pmatrix}
\end{equation*}

$M \in \mathbb{R}^{ \cin n^2 \times  \cin n^2}$

$M = A^\dag A$
\begin{equation*}
M =
\begin{pmatrix}
\sum_{j=1}^{\cout} {D[j,1]}^\dag D[j,1] & \dots &  \sum_{j=1}^{\cout} {D[j,1]}^\dag D[j,\cin]  \\
\vdots & \ddots & \vdots \\
\sum_{j=1}^{\cout} {D[j,\cin]}^\dag D[j,1] & \dots &  \sum_{j=1}^{\cout} {D[j,\cin]}^\dag D[j,\cin]  \\
\end{pmatrix}
\end{equation*}

%$||A||_2^2 = \sup_{||w||_2 = 1} ||Aw||_2^2 = \sup_{||w||_2 = 1} w^\top A^\top A w$ \\
%$||A||_2^2 = ||A^\top A||_2 = ||M||_2$

We have that $\sigma_1(A)^2 = \sigma_1(M)$

We apply Lemma \ref{lemma:concat_singular_value} on  $M$ we get another bound :

\begin{prop}
\label{bound:version_two}
$$
\sigma_1(A) \leq \sqrt[4]{ \max_{i \leq n^2} \left( \sum_{p=1}^{\cin} \sum_{i=1}^{\cin} 
\left| \sum_{j=1}^{\cout} {D[j,p]}^\dag D[j,i] \right|^2 \right)_{i}}$$
\end{prop}

\begin{proof} 
$M[p]$ a row of  $M$, 
$$M[p] = (\sum_{j=1}^{f} {D[j,p]}^\top D[j,1],  \sum_{j=1}^{f} {D[j,p]}^\top D[j,2],  \dots,  \sum_{j=1}^{f} {D[j,p]}^\top D[j,c] )$$


$\sigma_1(M[p])^2 = \lambda_1 (M[p] M[p]^\dag) $

$M[p] M[p]^\dag = \sum_{i=1}^{c} 
(\sum_{j=1}^{f} {D[j,p]}^\dag D[j,i]) (\sum_{j=1}^{f} {D[j,p]}^\dag D[j,i])^\dag$

$M[p] M[p]^\dag = \sum_{i=1}^{c} 
|\sum_{j=1}^{f} {D[j,p]}^\dag D[j,i])|^2$

$\sigma_1(M[p])^2 = \lambda_1 (\sum_{i=1}^{c} 
|\sum_{j=1}^{f} {D[j,p]}^\dag D[j,i])|^2) $

$\sigma_1(M[p])^2 = \max _{i \leq n^2} (\sum_{i=1}^{c} 
|\sum_{j=1}^{f} {D[j,p]}^\dag D[j,i])|^2)_{ii} $

with Lemma \ref{lemma:concat_singular_value} :
$\sigma_1(M)^2 \leq \sum_{p=1}^{c} \sigma_1(M[p])^2$.

$\sigma_1(M)^2 \leq \sum_{p=1}^{c} \max _{i \leq n^2} (\sum_{i=1}^{c} 
|\sum_{j=1}^{f} {D[j,p]}^\dag D[j,i])|^2)_{ii}$

$\sigma_1(M) \leq \sqrt{\sum_{p=1}^{c} \max _{i \leq n^2} (\sum_{i=1}^{c} 
|\sum_{j=1}^{f} {D[j,p]}^\dag D[j,i])|^2)_{ii}}$

$\sigma_1(A) \leq \sqrt[4]{\sum_{p=1}^{c} \max _{i \leq n^2} (\sum_{i=1}^{c} 
|\sum_{j=1}^{f} {D[j,p]}^\dag D[j,i])|^2)_{ii}}$

\end{proof}

\section{draft proof convergence to remove later}

\begin{proof}
we have a linear convergence rate for this bound, first: \\
\begin{equation*}
    \norm{\gamma}_\infty \leq \norm{\gamma}_p
\end{equation*}
for $q \leq p$
\begin{align*}
    \norm{\gamma}_p &= \left({\sum_i |\gamma_i|^p}\right)^{1/p} \\
    \norm{\gamma}_p &= \left(\sum_i |\gamma_i|^{p-q}|\gamma_i|^{q}\right)^{1/p} \\
    \norm{\gamma}_p &\leq \norm{\gamma}_\infty \left(\sum_i 
    \left(
    \frac{|\gamma_i|}{\norm{\gamma}_\infty}
    \right)^{q}
    \right)^{1/p} \\
\end{align*}

\begin{align*}
    \norm{\gamma}_p - \norm{\gamma}_\infty &\leq
      \norm{\gamma}_\infty ~ 
    \left( ~ 
    \left(
            \sum_i 
            \left(
            \frac{|\gamma_i|}{\norm{\gamma}_\infty}
            \right)^{q} 
            \right)^{\frac{1}{p}} - 1 
    \right) \\
    &\leq \norm{\gamma}_\infty ~ 
    \left| C^{\frac{1}{p}} -1 ~\right|
\end{align*}

\begin{align*}
    \left| C^{\frac{1}{p}} -1 ~\right| \underset{p\to +\infty}{=} \frac{\log(C)}{p} + O(\frac{1}{p^2})
\end{align*}
\end{proof}


\section{old part expressing conv}


For all $1 \leq u \leq n$, $\circm{K_{i,j,u}}$ is a circulant matrix and it is related to the discrete Fourier transform  : 

$\circm{K_{i,j,u}} = \frac{1}{n} F^T \diag{(F K_{i,j,u})} F$.
Then each $A_{ij}$ is a circulant doubly matrix and can also be diagonalized with the Hermitian matrices $F \otimes F$ like so : 
$A_{ij}= \frac{1}{n^2} (F \otimes F) \diag{(\vect{\Tilde{K}_{i,j}})} (F \otimes F)^\dag$. Diagonalize each $A_{i,j}$ would give  a block matrix A, where each block $A_{i,j}$ is diagonal.
Fourier transform diagonalizes circulant structure in matrix.

\blaise{avant fourier}

To pass from matrix $A$ to matrix $C$ is a reshape operation and is described in Figure~\ref{fig:reshape_kernel_cincout}. Each spatial pixel is grouped across channel dimension into matrices of size $\cout \times \cin$. It represents the same convolution operation thus:


$C$ is a doubly block circulant matrix where entries are $\cout \times \cin$ matrices. The Fourier transform diagonalizes the circulant structure and gives a block diagonal matrix where each block diagonal $G$ is a $\cout \times \cin$ matrices. There are $n^2$ of such blocks. This matrix structure is more convenient to derive a bound on Lipschitz constant.




%\begin{align*} C =R \begin{pmatrix}
%G_{1,1} & 0 & \dots & 0 \\
%0 & G_{1,2} & \dots & 0 \\
%\vdots & \vdots & \ddots & \vdots \\
%0 &  \dots &  0 & G_{n,n}
%\end{pmatrix} Q^\dag \end{align*}

\section{table training time and accuracies}
\begin{table}[h]\centering
\scriptsize
\begin{tabular}{lrrrrrr}\toprule
\textbf{Method} &Ours &Singla2021 &Araujo2021 &Baseline &Baseline WD \\\cmidrule{1-6}
\textbf{Accuracy(\%)} &93.79 &92.97 &92.3 &93.29 &93.3 \\\midrule
\textbf{Time per epoch (s)} &31.9 &38.4 &37.4 &11.4 &11.4 \\\midrule
\end{tabular}
\caption{Test accuracies from trainings on CIFAR-10 for baseline with and without weight decay (WD) and different regularizations.}
\label{tab:test_accuracies_method_reg_cifar10}
\end{table}

\section{Proof of Proposition \ref{prop:convergence_rate}}
\label{proof:convergence_rate}

\begin{defn}
Q-Linear and Q-Superlinear convergence.\\ 
     Suppose sequence $(u_t)_{t \in \mathbb{N}}$ converges to $u^*$, it converges Q-linearly if
    $\underset{t \to +\infty}{\text{lim}} \frac{|u_{n+1} - u^* |}{|u_{n} - u^* |} = \mu < 1$.
    It converges Q-superlinearly if $\mu = 0$.
    The number $\mu$ is called the rate of convergence. 

    We say that we have quadratic convergence if  $\underset{t \to +\infty}{\text{lim}} \frac{|u_{n+1} - u^* |}{|u_{n} - u^* |^2} = 0$
    \blaise{est ce qu'on peut dire qu'on a une convergence quadratique ? demander Clément et Yann}
\end{defn}

\begin{prop*}
If $\left|\gamma_2\right| < \left|\gamma_1\right|$ the convergence is Q-superlinear ($\forall \epsilon > 0$, order of convergence $q > 2 - \epsilon$), else it is Q-linear of rate $\frac{1}{2}$.
\end{prop*}

\begin{proof}
For $t \geq 1$, we have:
\begin{align*}
    \norm{\gamma}_{t} - \norm{\gamma}_{\infty} 
   %&= \norm{\gamma}_{\infty}
   %\left(
   %\frac{\norm{\gamma}_{t}}{\norm{\gamma}_{\infty}} - 1
   %\right)\\
   &= \norm{\gamma}_{\infty}
   \left(
         \left(\sum_i 
                \frac{|\gamma_i|^t}
                {\norm{\gamma}_{\infty}^t}
          \right)^{1/t}
         - 1
   \right)\\
   &= \norm{\gamma}_{\infty}
   \left(
         \exp{ \left( \frac{1}{t}
                \log{\sum_i 
                \frac{|\gamma_i|^t}
                {\norm{\gamma}_{\infty}^t}}
          \right)}
         - 1
   \right)
\end{align*}
\begin{align*}
   \log{\sum_i \frac{|\gamma_i|^t}{\norm{\gamma}_{\infty}^t}} &= 
    \log{ \left( 1 + \alpha \right)} ~ \text{with} ~
    \alpha=\sum_{i \neq 1} 
    \frac{|\gamma_i|^t}
    {\norm{\gamma}_{\infty}^t} \underset{t\to +\infty}{\longrightarrow} 0\\
    \log{\sum_i \frac{|\gamma_i|^t}{\norm{\gamma}_{\infty}^t}} &\underset{t \to +\infty}{=} \alpha + o(\alpha^2)
\end{align*}
\begin{align*}
\norm{\gamma}_{t} - \norm{\gamma}_{\infty} &\underset{t \to +\infty}{=} \norm{\gamma}_{\infty}
   \left(
         (1 + \frac{1}{t} \alpha + o(\alpha^2)) -1
   \right)\\
   &\underset{t \to +\infty}{=} \frac{\norm{\gamma}_{\infty}}{t}
   \left(
         \alpha + o(\alpha^2)
   \right)
\end{align*}

Hence  
\begin{align*}
 \frac{\norm{\gamma}_{2^{t+1}} - \norm{\gamma}_{\infty}}
 {\norm{\gamma}_{2^{t}} - \norm{\gamma}_{\infty}} &
 \underset{t \to +\infty}{\sim}
 \frac{2^t}{2^{t+1}}
 \frac{\sum_{i \neq 1} 
        \frac{|\gamma_i|^{2^{t+1}}}
        {\norm{\gamma}_{\infty}^{2^{t+1}}}
      }
      {\sum_{i \neq 1} 
        \frac{|\gamma_i|^{2^t}}
        {\norm{\gamma}_{\infty}^{2^t}}
      }\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\frac{\norm{\gamma}_{2^{t+1}} - \norm{\gamma}_{\infty}}
     {\norm{\gamma}_{2^t} - \norm{\gamma}_{\infty}} &
     \underset{t \to +\infty}{\sim}
     \frac{\norm{\gamma}_{\infty}^{2^{t}}}{2\norm{\gamma}_{\infty}^{2^{t+1}}}
     \frac{\sum_{i \neq 1} 
            |\gamma_i|^{2^t} |\gamma_i|^{2^t}
          }
          {\sum_{i \neq 1} 
            |\gamma_i|^{2^t}
          }\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\frac{\norm{\gamma}_{2^{t+1}} - \norm{\gamma}_{\infty}}
     {\norm{\gamma}_{2^t} - \norm{\gamma}_{\infty}} &
     \underset{t \to +\infty}{\sim}
     \frac{1}{2\norm{\gamma}_{\infty}^{2^{t}}}
     \frac{\sum_{i \neq 1} 
            |\gamma_i|^{2^t} |\gamma_i|^{2^t}
          }
          {\sum_{i \neq 1} 
            |\gamma_i|^{2^t}
          }\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
     \frac{1}{2\norm{\gamma}_{\infty}^{2^t}}
     \frac{\sum_{i \neq 1} 
            |\gamma_i|^{2^t}|\gamma_i|^{2^t}
          }
          {\sum_{i \neq 1} 
            |\gamma_i|^{2^t}
          } &\leq 
          \frac{|\gamma_2|^{2^t}}{2\norm{\gamma}_{\infty}^{2^t}} =
          \frac{1}{2}\left|\frac{\gamma_2}{\gamma_1}\right|^{2^t}
          \underset{t\to +\infty}{\longrightarrow} 0
 \end{align*}

If $\left|\gamma_2\right| < \left|\gamma_1\right|$, then $\frac{1}{2}\left|\frac{\gamma_2}{\gamma_1}\right|^{2^t}
          \underset{t\to +\infty}{\longrightarrow} 0$ .
\end{proof}

\section{tableau resnet 18 convs}
\begin{table*}[tb]\centering
\scriptsize
\begin{tabular}{lrrrrrrrrrrrr}\toprule
\textbf{Filter Shape} &\multicolumn{5}{c}{\textbf{Lipschitz Bound}} & &\multicolumn{5}{c}{\textbf{Running Time (s)}} \\\cmidrule{2-6}\cmidrule{8-12}
&Ours &Singla2021 &Araujo2021 &Sedghi2019 &Ryu2019 & &Ours &Singla2021 &Araujo2021 &Sedghi2019 &Ryu2019 \\\cmidrule{2-6}\cmidrule{8-12}
64 $\times$ 3 $\times$ 7 $\times$ 7 &15.91 &28.89 &22.25 &15.91 &15.91 & &0.0024 &0.0507 &0.0003 &18.06 &0.7579 \\\cmidrule{1-6}\cmidrule{8-12}
64 $\times$ 64 $\times$ 3 $\times$ 3 & 6 &9.32 &17.59 &6 &6 & &0.0014 &0.0264 &0.0003 &7.47 &1.07 \\\cmidrule{1-6}\cmidrule{8-12}
64 $\times$ 64 $\times$ 3 $\times$ 3 &5.34 &6.28 &15.31 &5.34 &5.33 & &0.0015 &0.025 &0.0012 &7.29 &1.07 \\\cmidrule{1-6}\cmidrule{8-12}
64 $\times$ 64 $\times$ 3 $\times$ 3 &7 &8.71 &16.46 &7 &7 & &0.0011 &0.026 &0.0003 &7.27 &1.08 \\\cmidrule{1-6}\cmidrule{8-12}
64 $\times$ 64 $\times$ 3 $\times$ 3 &3.82 &5.40 & 13.74 &3.81 &3.82 & &0.0014 &0.025 &0.0003 &7.19 &1.08 \\\cmidrule{1-6}\cmidrule{8-12}
128 $\times$ 64 $\times$ 3 $\times$ 3 & 4.71 &5.98 &16.35 &4.71 &4.7 & &0.0014 &0.026 & 0.0012 & 9 & 0.473 \\\cmidrule{1-6}\cmidrule{8-12}
128 $\times$ 128 $\times$ 3 $\times$ 3 &5.72 &7.21 & 23.58 &5.72 &5.72 & &0.0011 &0.026 &0.0013 &4.85 &0.78 \\\cmidrule{1-6}\cmidrule{8-12}
128 $\times$ 64$\times$ 1 $\times$ 1 &1.91 &1.91 &6.39 &1.91 &1.91 & &0.0014 & 0.0333 &0.0001 &9.25 &0.042 \\\cmidrule{1-6}\cmidrule{8-12}
128 $\times$ 128 $\times$ 3 $\times$ 3 &4.41 &6.78 & 21.93 &4.4 &4.41 & &0.0011 &0.026 &0.0003 &4.844 &0.78 \\\cmidrule{1-6}\cmidrule{8-12}
128 $\times$ 128 $\times$ 3 $\times$ 3 &4.89 &7.57 & 19.79 &4.89 & 4.88 & & 0.0014 & 0.027 &0.0004 &4.78 & 0.78 \\\cmidrule{1-6}\cmidrule{8-12}
256 $\times$ 128 $\times$ 3 $\times$ 3 &7.39 &8.45 &35.86 & 7.39 &7.38 & &0.0014 &0.026 &0.0017 &5.36 & 0.46 \\\cmidrule{1-6}\cmidrule{8-12}
256 $\times$ 256 $\times$ 3 $\times$ 3 &6.58 &8.03 &37.98 &6.58 &6.57 & &0.0014 &0.026 &0.0025 &3.46 &0.85 \\\cmidrule{1-6}\cmidrule{8-12}
256 $\times$ 128$\times$ 1 $\times$ 1 &1.21 &1.21 &5.97 &1.21 & 1.21 & &0.0014 & 0.036 &0.0001 &5.96 & 0.04 \\\cmidrule{1-6}\cmidrule{8-12}
256 $\times$ 256 $\times$ 3 $\times$ 3 &6.36 &7.57 &30.07 &6.36 &6.35 & &0.001 &0.026 &0.0004 &3.48 &0.85 \\\cmidrule{1-6}\cmidrule{8-12}
256 $\times$ 256 $\times$ 3 $\times$ 3 & 7.68 &9.17 &29.19 & 7.68 &7.67 & & 0.0011 &0.027 &0.0004 &3.48 & 0.85 \\\cmidrule{1-6}\cmidrule{8-12}
512 $\times$ 256 $\times$ 3 $\times$ 3 &9.99 &11 &46.24 &9.99 &9.92 & &0.0011 &0.026 &0.004 &3.55 &0.45 \\\cmidrule{1-6}\cmidrule{8-12}
512 $\times$ 512 $\times$ 3 $\times$ 3 &9.09 &10.45 &47.59 &9.09 &9.04 & &0.0014 &0.026 &0.0001 &2.8 &0.79 \\\cmidrule{1-6}\cmidrule{8-12}
512 $\times$ 256 $\times$ 1 $\times$ 1 &2.05 &2.03 &11.87 &2.05 &2.05 & &0.0012 &0.024 &0.0001 &3.77 &0.052 \\\cmidrule{1-6}\cmidrule{8-12}
512 $\times$ 512 $\times$ 3 $\times$ 3 &17.6 &18.37 &59.04 &17.60 &17.5 & &0.001 &0.027 &0.0005 &2.79 &0.79 \\\cmidrule{1-6}\cmidrule{8-12}
512 $\times$ 512 $\times$ 3 $\times$ 3 &7.48 & 7.6 & 57.33 &7.48 &7.43 & &0.0014 &0.027 &0.0006 &2.83 &0.79 \\
\bottomrule
\end{tabular}
\caption{Comparison of Lipschitz bounds for all convolutional layers ResNet18, reference for real Lipschitz bound is given by \cite{Ryu19Plug} method.}
\label{tab:lipschitz_resnet18}
\end{table*}



\section{proof v1 convergence}
\begin{align*}
    \text{We define} \ \ \
    \epsilon_t &=\left(\sum_{i=1}^m \left|\frac{\gamma_i}{\gamma_1}\right|^{2^{t}} \right)^{2^{-t}} - 1
    \\
    \epsilon_t &= \exp{
        \left(
            2^{-t}
            \log\left(\sum_{i=1}^m \left|\frac{\gamma_i}{\gamma_1}\right|^{2^{t}} \right) 
        \right)}
        - 1 \\
         \epsilon_t &= \exp{
        \left(
            2^{-t}
            \log\left(1 + \sum_{i=2}^m \left|\frac{\gamma_i}{\gamma_1}\right|^{2^{t}} \right) 
        \right)}
        - 1 \\
        \text{Using series expansion:} \ \
        \epsilon_t &\underset{t \to +\infty}{=} \exp{
        \left(
            2^{-t}
            \left( \alpha + o(\alpha^2) \right) 
        \right)}
        - 1 \\
        \epsilon_t &\underset{t \to +\infty}{=} 
            2^{-t} \alpha + o(2^{-t}\alpha^2)
\end{align*}
with $\alpha = \sum_{i=2}^m \left|\frac{\gamma_i}{\gamma_1}\right|^{2^{t}} \underset{t\to +\infty}{\longrightarrow} 0$.

For $q > 0$,
\begin{align*}
    \frac{\epsilon_{t+1}}{\epsilon_{t}^q} &\underset{t \to +\infty}{\sim} 
    \frac
    {2^{-(t+1)}
        \sum_{i=2}^m \left|\frac{\gamma_i}{\gamma_1}\right|^{2^{t+1}}
    }
    {2^{-tq} 
    \left(
        \sum_{i=2}^m \left|\frac{\gamma_i}{\gamma_1}\right|^{2^{t}}
    \right)^q}\\
    \frac{\epsilon_{t+1}}{\epsilon_{t}^q} &\underset{t \to +\infty}{\sim} 
    2^{t(q -1) - 1}
    \frac
    {
        \left|\frac{\gamma_2}{\gamma_1}\right|^{2^{t+1}}
    }
    { 
        \left|\frac{\gamma_2}{\gamma_1}\right|^{q2^{t}}
    }\\
    \frac{\epsilon_{t+1}}{\epsilon_{t}^q} &\underset{t \to +\infty}{\sim} 
    2^{t(q -1) - 1}
    \left|\frac{\gamma_2}{\gamma_1}\right|^{2^{t}(2 - q)}
\end{align*}

If $|\gamma_2| = |\gamma_1|$, convergence is Q-linear ($q=1$) of rate $\frac{1}{2}$. \\
Else, when $|\gamma_2| < |\gamma_1|$, for $0 < q < 2$,
$\underset{t \to +\infty}{\lim} \frac{\epsilon_{t+1}}{\epsilon_{t}^q} = 0$, hence convergence is Q-quadratic.


\section{proof convergence V2 qui marche pas}

\begin{align*}
    \text{We define} \ \ \
    \epsilon_t &=\left(\sum_{i=1}^m \left|\frac{\gamma_i}{\gamma_1}\right|^{2^{t}} \right)^{2^{-t}} - 1
    \\
    \epsilon_t &= \exp{
        \left(
            2^{-t}
            \log\left(\sum_{i=1}^m \left|\frac{\gamma_i}{\gamma_1}\right|^{2^{t}} \right) 
        \right)}
        - 1 \\
         \epsilon_t &= \exp{
        \left(
            2^{-t}
            \log\left(1 + \sum_{i=2}^m \left|\frac{\gamma_i}{\gamma_1}\right|^{2^{t}} \right) 
        \right)}
        - 1 \\
        \text{Using series expansion:} \ \
        \epsilon_t &\underset{t \to +\infty}{=} \exp{
        \left(
            2^{-t}
            \left( \alpha + o(\alpha^2) \right) 
        \right)}
        - 1 \\
        \epsilon_t &\underset{t \to +\infty}{=} 
            2^{-t} \alpha + o(2^{-t}\alpha^2)
\end{align*}
with $\alpha = \sum_{i=2}^m \left|\frac{\gamma_i}{\gamma_1}\right|^{2^{t}} \underset{t\to +\infty}{\longrightarrow} 0$.

Computing ratio $\epsilon_{t+1} / \epsilon_{t}^q$ for $q=2$:

\begin{align*}
    \epsilon_{t+1} \underset{t \to +\infty}{\sim} 
    2^{-(t+1)}
        \sum_{i=2}^m \left|\frac{\gamma_i}{\gamma_1}\right|^{2^{t+1}}
\end{align*}
and

\begin{align*}
    \epsilon_{t}^2 &= 
    1 + 
    \left(\sum_{i=1}^m \left|\frac{\gamma_i}{\gamma_1}\right|^{2^{t}} \right)^{2^{-t+1}} 
    - 2 \left(\sum_{i=1}^m \left|\frac{\gamma_i}{\gamma_1}\right|^{2^{t}} \right)^{2^{-t}}  \\
    %%%%%%%%%%%%%%%
    \epsilon_{t}^2 &\underset{t \to +\infty}{=}  
    2^{-t +1}
        \sum_{i=2}^m \left|\frac{\gamma_i}{\gamma_1}\right|^{2^{t}} 
    - 2^{-t +1}
        \sum_{i=2}^m \left|\frac{\gamma_i}{\gamma_1}\right|^{2^{t}}
    + o(2^{-t+1} \alpha) \\
    %%%%%%%%%%%%%%%%
    \epsilon_{t}^2 &\underset{t \to +\infty}{\sim} 
    2^{-t +1}
        \sum_{i=2}^m \left|\frac{\gamma_i}{\gamma_1}\right|^{2^{t}} 
    - 2^{-t +1}
        \sum_{i=2}^m \left|\frac{\gamma_i}{\gamma_1}\right|^{2^{t}}
\end{align*}

\begin{align*}
    \frac{\epsilon_{t+1}}{\epsilon_{t}^2} &\underset{t \to +\infty}{=} 
    \frac
    {
    2^{-(t+1)}
        \sum_{i=2}^m \left|\frac{\gamma_i}{\gamma_1}\right|^{2^{t+1}} + o(2^{-(t+1)} \alpha^2)
    }
    {
    \left(
    \left(\sum_{i=1}^m \left|\frac{\gamma_i}{\gamma_1}\right|^{2^{t}} \right)^{2^{-t}} - 1
    \right)^2
    }\\
    %%%%%%%%%%%%%%%%%%%%%%%%%
     \frac{\epsilon_{t+1}}{\epsilon_{t}^2} &\underset{t \to +\infty}{=} 
    \frac
    {2^{-(t+1)}
        \sum_{i=2}^m \left|\frac{\gamma_i}{\gamma_1}\right|^{2^{t+1}} + o(2^{-(t+1)} \alpha^2)
    }
    {
    1 + 
    \left(\sum_{i=1}^m \left|\frac{\gamma_i}{\gamma_1}\right|^{2^{t}} \right)^{2^{-(t+1)}} 
    - 2 \left(\sum_{i=1}^m \left|\frac{\gamma_i}{\gamma_1}\right|^{2^{t}} \right)^{2^{-t}} 
    }\\
    %%%%%%%%%%%%%%%%%%%%%%%%%
     \frac{\epsilon_{t+1}}{\epsilon_{t}^2} &\underset{t \to +\infty}{=} 
    \frac
    {2^{-(t+1)}
        \sum_{i=2}^m \left|\frac{\gamma_i}{\gamma_1}\right|^{2^{t+1}} + o(2^{-(t+1)} \alpha^2)
    }
    {
    1 + 
    \left(\sum_{i=1}^m \left|\frac{\gamma_i}{\gamma_1}\right|^{2^{t}} \right)^{2^{-(t+1)}} 
    - 2^{-t +1}
        \sum_{i=2}^m \left|\frac{\gamma_i}{\gamma_1}\right|^{2^{t}}
    }\\
\end{align*}

If $|\gamma_2| = |\gamma_1|$, convergence is Q-linear ($q=1$) of rate $\frac{1}{2}$. \\
Else, when $|\gamma_2| < |\gamma_1|$, 
$\underset{t \to +\infty}{\lim} \frac{\epsilon_{t+1}}{\epsilon_{t}^q} = 0$, hence convergence is Q-quadratic.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Stabilization of GANs by spectral normalization}
% https://github.com/pfnet-research/sngan_projection

Generative adversarial networks (GANs) are very difficult to train and prone to mode collapse due to sharp discriminator's gradient [ref].
Bounding the Lipschitz constant of the discriminator improves training stability [ref]. 
We use the same formulation for the GAN problem as in \cite{miyato2018spectral}, use their experimental framework and compare with their method spectral normalizaton (SN) using PI.
To show effectiveness of Gram iteration for spectral normalization we present in [TABLE] the results IS and FID [ref] of different training setting and how our method can handle more aggressive training setting than SN (learning rate, etc).
\blaise{argument marketing: simple spectral norm, sans tricks. TODO Faire la table}

\section{Algo qui marche pas}
\blaise{pb on perd la prop de borne}
\begin{algorithm}[h]
\caption{: Gram\_iteration\_actual$(G, t_\text{max})$}
\label{algo:gram_iteration_actual}
\begin{algorithmic}[1]
  \STATE \textbf{Inputs} matrix: $G$, iterations: $t_\text{max}$
  \STATE $G_1 \gets G$ 
  \STATE \textbf{for} $1 \ldots t_\text{max}$
    \STATE \quad $G \gets G^\dag G$
    \STATE \quad $G \gets G/\norm{G}_F$
  \STATE $\sigma_1 \gets \norm{G_1 G}_F$
  \STATE \textbf{return} $\sigma_1$
\end{algorithmic}
\end{algorithm}


\section{old table 2}
\begin{table*}[tb]\centering
\sisetup{%
    table-align-uncertainty=true,
    separate-uncertainty=true,
    detect-weight=true,
    detect-inline-weight=math
  }
\scriptsize
\scriptsize
\begin{tabular}
    {
    l
     l%S[table-format=2.2]%r
     l
     l%S[table-format=2.2]%r
     l%S[table-format=2.2]%r
     l%S[table-format=2.2]%r
     l%S[table-format=2.2]%r
     l%S[table-format=2.2]%r
     l%S[table-format=2.2]%r
     l%S[table-format=2.2]%r
     l%S[table-format=2.2]%r
     l%S[table-format=2.2]%r
    }
\toprule
\textbf{Model} &\multicolumn{4}{c}{\textbf{Ratio of Network Lipschitz Bound}} & &\multicolumn{5}{c}{\textbf{Total Running Time (s)}} \\\cmidrule{1-5}\cmidrule{7-11}
&Ours &\citeauthor{singla2021fantastic} &\citeauthor{araujo2021lipschitz} &\citeauthor{sedghi2019singular} & &Ours &\citeauthor{singla2021fantastic} &\citeauthor{araujo2021lipschitz} &\citeauthor{sedghi2019singular} &\citeauthor{Ryu19Plug} \\\cmidrule{2-5}\cmidrule{7-11}
VGG16 &$1.14 \pm 0.02$ & $23.90 \pm 6.8$ & $4.88\mathrm{e}{+9}\pm 4.83\mathrm{e}{+9}$ &$1.14 \pm 0.02$ & &0.015 &0.32 &0.02 &525 &0.40 \\\cmidrule{1-5}\cmidrule{7-11}
%
VGG19 &$1.16  \pm 0.005$ & $30.63 \pm 0.3$ & $9.70\mathrm{e}{+9}\pm 4.84\mathrm{e}{+7}$ & $1.16 \pm 0.005$ & &0.018 &0.39 &0.02 &639 &0.52 \\\cmidrule{1-5}\cmidrule{7-11}
%
ResNet18 &$1.47 \pm 0.007$ &$87.93 \pm 0.88$ &$3.03\mathrm{e}{+10} \pm 1.56\mathrm{e}{+8}$ &$1.47 \pm 0.007$ & &0.013 &0.45 &0.0161 &185 &1.02 \\\cmidrule{1-5}\cmidrule{7-11}
%
ResNet34 &$1.82 \pm 0.35$ & $4982 \pm 4894$ &$7.86\mathrm{e}{+21} \pm 7.86\mathrm{e}{+21}$ &$2.15 \pm 0.35$ & &0.026 &0.88 &0.03 &237 &1.82 \\\cmidrule{1-5}\cmidrule{7-11}
%
ResNet50 &$1.68 \pm 0.35$ &$3338 \pm 4622$ &$6.66\mathrm{e}{+31} \pm 9.42\mathrm{e}{+31}$ &$1.67 \pm 0.35$ & &0.039 &1.28 &0.05 &377 &1.67 \\\cmidrule{1-5}\cmidrule{7-11}
%
ResNet101 &$1.74 \pm 0.32$ &$4026\pm 4178$ &$6.55\mathrm{e}{+64}\pm 1.13\mathrm{e}{+65}$ &$1.74\pm 0.32$ & &0.073 &2.60 &0.10 &551 &1.74 \\\cmidrule{1-5}\cmidrule{7-11}
%
ResNet152 &$1.92 \pm 0.46$ &$8.39\mathrm{e}{+4} \pm 1.60\mathrm{e}{+5}$ &$2.85\mathrm{e}{+96} \pm 5.71\mathrm{e}{+96}$ &$1.92 \pm 0.46$ & &0.109 &3.93 &0.12 &725 &6.17 \\
\bottomrule
\end{tabular}
\caption{Comparison of network bound Lipschitz ratio with standard deviation for several CNNs, reference for computing the ratio is the bound given by \cite{Ryu19Plug} method. Using Equation~\ref{eq:prod_lip_bound}, an overall Lipschitz constant bound $B_{\text{method}}$ is obtained for different method. Ratio of network Lipschitz bound is defined as : $\frac{B_{\text{method}}}{B_{\text{Ryu2019}}}$. Results are averaged over 100 runs. Ratio standard deviations of ours, \cite{araujo2021lipschitz} and \cite{sedghi2019singular} are induced by \cite{Ryu19Plug} method.
}
\label{tab:lipschitz_product_ratio_ryu}
\end{table*}

\section{old tabel 1}
\begin{table*}[tb]\centering
\sisetup{%
    table-align-uncertainty=true,
    separate-uncertainty=true,
    detect-weight=true,
    detect-inline-weight=math
  }
\scriptsize
\scriptsize
\begin{tabular}
    {
    l
     l%S[table-format=2.2]%r
     l
     l%S[table-format=2.2]%r
     l%S[table-format=2.2]%r
     l%S[table-format=2.2]%r
     l%S[table-format=2.2]%r
     l%S[table-format=2.2]%r
     l%S[table-format=2.2]%r
     l%S[table-format=2.2]%r
     l%S[table-format=2.2]%r
     l%S[table-format=2.2]%r
    }
\toprule
\textbf{Model} &\multicolumn{4}{c}{\textbf{Ratio of Network Lipschitz Bound}} & &\multicolumn{5}{c}{\textbf{Total Running Time (s)}} \\\cmidrule{1-5}\cmidrule{7-11}
&Ours &\citeauthor{singla2021fantastic} &\citeauthor{araujo2021lipschitz} &\citeauthor{sedghi2019singular} & &Ours &\citeauthor{singla2021fantastic} &\citeauthor{araujo2021lipschitz} &\citeauthor{sedghi2019singular} &\citeauthor{Ryu19Plug} \\\cmidrule{2-5}\cmidrule{7-11}
VGG16 &$1.14 \pm 0.02$ & $23.90 \pm 6.8$ & $4.88\mathrm{e}{+9}\pm 4.83\mathrm{e}{+9}$ &$1.14 \pm 0.02$ & &0.015 &0.32 &0.02 &525 &0.40 \\\cmidrule{1-5}\cmidrule{7-11}
%
VGG19 &$1.16  \pm 0.005$ & $30.63 \pm 0.3$ & $9.70\mathrm{e}{+9}\pm 4.84\mathrm{e}{+7}$ & $1.16 \pm 0.005$ & &0.018 &0.39 &0.02 &639 &0.52 \\\cmidrule{1-5}\cmidrule{7-11}
%
ResNet18 &$1.47 \pm 0.007$ &$87.93 \pm 0.88$ &$3.03\mathrm{e}{+10} \pm 1.56\mathrm{e}{+8}$ &$1.47 \pm 0.007$ & &0.013 &0.45 &0.0161 &185 &1.02 \\\cmidrule{1-5}\cmidrule{7-11}
%
ResNet34 &$1.82 \pm 0.35$ & $4982 \pm 4894$ &$7.86\mathrm{e}{+21} \pm 7.86\mathrm{e}{+21}$ &$2.15 \pm 0.35$ & &0.026 &0.88 &0.03 &237 &1.82 \\\cmidrule{1-5}\cmidrule{7-11}
%
ResNet50 &$1.68 \pm 0.35$ &$3338 \pm 4622$ &$6.66\mathrm{e}{+31} \pm 9.42\mathrm{e}{+31}$ &$1.67 \pm 0.35$ & &0.039 &1.28 &0.05 &377 &1.67 \\\cmidrule{1-5}\cmidrule{7-11}
%
ResNet101 &$1.74 \pm 0.32$ &$4026\pm 4178$ &$6.55\mathrm{e}{+64}\pm 1.13\mathrm{e}{+65}$ &$1.74\pm 0.32$ & &0.073 &2.60 &0.10 &551 &1.74 \\\cmidrule{1-5}\cmidrule{7-11}
%
ResNet152 &$1.92 \pm 0.46$ &$8.39\mathrm{e}{+4} \pm 1.60\mathrm{e}{+5}$ &$2.85\mathrm{e}{+96} \pm 5.71\mathrm{e}{+96}$ &$1.92 \pm 0.46$ & &0.109 &3.93 &0.12 &725 &6.17 \\
\bottomrule
\end{tabular}
\caption{Comparison of a network bound Lipschitz ratio with standard deviation for several CNNs, reference for computing the ratio is the bound given by \cite{Ryu19Plug} method. Using Equation~\ref{eq:prod_lip_bound}, an overall Lipschitz constant bound $B_{\text{method}}$ is obtained for different methods. Ratio of network Lipschitz bound is defined as : $\frac{B_{\text{method}}}{B_{\text{Ryu2019}}}$. Results are averaged over 100 runs. Ratio standard deviations of ours, \cite{araujo2021lipschitz} and \cite{sedghi2019singular} are induced by \cite{Ryu19Plug} method.
}
\label{tab:lipschitz_product_ratio_ryu}
\end{table*}

==> sections/conv_old.tex <==


\subsection*{Notations}

A matrix is defined by its elements as $A = [A_{i,j}]_{i,j}$, with 1-indexing.
For a tensor $K \in \mathbb{R}^{c \times c \times n \times n}$, $K_{k}$ denotes the sub tensor $K_{k, : , : , :}$ and $K_{k,l}$ denotes $K_{k, l , : , :}$ a $n \times n$ matrix.
We denote the usual matrix product as $AB$,
and the Kronecker product as $A \otimes B$.
%We use $*$ to represent convolution product.
Hermitian transpose of matrix $A$ is noted as $A^\dag = \overline{{A^\top}} $.
The set of singular values of $A$ is denoted $\sigma(A) = \{ \sigma_i(A) \}_{i=1}^m$, using the decreasing order indexation convention $\sigma_1 \geq \sigma_i$.
%
The 2D Fourier transform for a matrix $X \in \mathbb{R}^{n \times n}$ is $\tilde{X} = F^\top X F \in \mathbb{C}^{n \times n}$, where 
$F = [e^{-2uvk\pi/n}]_{1 \leq u,v \leq n} 
%\in \mathbb{C}^{n \times n}
$ is the Fourier transform matrix. When $X$ is vectorized, $\vect{\Tilde{X}} = (F \otimes F) \vect{X}$. 
%If $X \in \mathbb{R}^{n}$, $\Tilde{X} = F X$.
%If $X \in \mathbb{R}^{n \times n}$, $\Tilde{X} = F^\top X F \in \mathbb{C}^{n \times n}$.
%If $X \in \mathbb{R}^{\cout \times \cin \times n \times n}$, $\tilde{X} = [F^\top X_{i,j} F]_{i,j}$.
 
For a vector $a = [a_i]_{1 \leq i \leq m}  \in \mathbb{R}^{m}$,
$\diag(a) \in \mathbb{R}^{m \times m}$
is the matrix with $a$ on the diagonal,
and $\circm{a} \in \mathbb{R}^{m \times m}$ is the circulant matrix:
\begin{equation*}
\circm{a} = \begin{pmatrix}
a_{1} & a_{2} & \dots & a_{m} \\
a_{m} & a_{1} & \dots & a_{m-1} \\
\vdots & \vdots & \ddots & \vdots \\
a_{2} & a_{3} & \dots & a_{1}
\end{pmatrix} \ .
\end{equation*}
%In the same manner, $\bdiag(A_1, \dots, A_m)$ represents a block diagonal matrix.
%Likewise we define block circulant matrix  $\circm{A_1, \dots, A_m}$, where $A_i$ are matrices. When $A_k$ are circulant matrices, we call it a doubly block circulant matrix, \cite{goodfellow2016deep}.

%\paragraph{Eigenvalues} Denote the sorted eigenvalues $\lambda_1 \geq \lambda_2 \geq   \dots \geq \lambda_n$.




% \subsection{Formulations of convolutional layer}
% \label{subsection:expression_conv_layers}

Let be $X \in \mathbb{R}^{\cin \times n \times n}$ the input and $Y \in \mathbb{R}^{\cout \times n \times n}$ the output of the convolution of layer defined by filter $K \in \mathbb{R}^{\cout \times \cin \times k \times k}$. We assume that $Y$ has the same spatial size as $X$ for convenience.
As in \cite{yi2020asymptotic}, we consider the case where stride equals 1; see \cite{senderovich2022towards} for case where stride $> 1$.

For an output channel $1\leq i \leq \cout$ and an output pixel $1 \leq u,v \leq n$, the output of a convolution layer can be written:
\begin{equation}
\label{eq:conv_kernel}
Y_{i,u,v} = \sum_{j=1}^\cin \sum_{u'=1}^n \sum_{v'=1}^n X_{j, u+u', v+v'} K_{i, j, u', v'} \ ,
\end{equation}
where $K_{i, j, u', v'}=0$ if $u',v' \geq k$, \ie $K$ is zero-padded to match input spatial size.

The convolution product between a 4D filter and a
3D input $X$ can be expressed as a matrix vector product, where the matrix $A$ is the concatenation row and column wise of doubly block Toeplitz matrices \cite{jain1989fundamentals}. The structure of $A$ accounts for the weight sharing property of convolutional layer cast as dense layer.
After input vectorization, we have
$\vect{Y} = A ~ \vect{X}$, with $A \in \mathbb{R}^{\cout n^2 \times \cin n^2}$ defined as:
\begin{equation*}
A = 
\begin{pmatrix}
A_{1,1} & \dots & A_{1,\cin} \\
% A_{2,1} & \dots & A_{2, \cin} \\
\vdots &  & \vdots \\
A_{\cout,1} & \dots & A_{\cout, \cin}
\end{pmatrix} \ .
\end{equation*}
For $1 \leq j \leq \cout$ and $1 \leq i \leq \cout$,
each $A_{i,j}$ is a  doubly block Toeplitz matrix depending of $K_{i,j}$ \cite{yi2020asymptotic}, as illustrated in \cite{wang2020orthogonal}, $A$ is referred to as multi-block doubly block Toeplitz matrix.
Hence, estimating the largest singular value of the convolution is equivalent to compute $\sigma_1(A)$. In practice computing this quantity is not tractable.

Fourier transform diagonalizing circulant matrices, 
it reduces computation complexity to approximate $A$ as a circular convolution $B$.
We consider output spatial size equals to input spatial size for sake of simplicity, general case being studied in \cite{yi2020asymptotic}. Now, $\vect{Y} = B ~ \vect{X}$, with $B = [B_{i,j}]_{i,j}$.
In this setting, each $B_{i,j} \in \mathbb{R}^{n \times n}$ is a doubly block circulant matrix of kernel $K_{i,j}$, it means that $B_{i,j}$ is a matrix circulant per block  and each block itself is a circulant matrix: 
\begin{align*}
    B_{i,j} =
    \begin{pmatrix}
    \text{circ}(K_{i,j,1}) & \text{circ}(K_{i,j,2}) & \dots & \text{circ}(K_{i,j,n}) \\
    \text{circ}(K_{i,j,n}) & \text{circ}(K_{i,j,1}) & \dots & \text{circ}(K_{i,j,n-1}) \\
    \vdots & \vdots & \ddots & \vdots \\
    \text{circ}(K_{i,j,2}) & \text{circ}(K_{i,j,3}) & \dots & \text{circ}(K_{i,j,1}) \\
    \end{pmatrix}
\end{align*}
$B$ is a multi-block doubly circulant matrix, \cite{yi2020asymptotic}. 2D Fourier transform $F \otimes F$ diagonalizes doubly block circulant matrices $B_{i,j}$, their singular values are the $\{ \Tilde{K}_{i,j, u,v} ~|~ 1 \leq u, v \leq n\}$.

% \blaise{est ce que $\sigma_1(A) \leq \sigma_1(B) ?$ seems true \cite{yi2020asymptotic}}

\begin{prop}[\citet{jain1989fundamentals}]
For a doubly block circulant matrix $B_{i,j} \in \mathbb{R}^{n^2 \times n^2}$ generated from kernel $K_{i,j} \in \mathbb{R}^{n \times n}$,
\begin{equation*}
B_{i,j} = \frac{1}{n^2}(F \otimes F)^\dag \diag(\vect{\tilde{K}_{i,j}}) (F \otimes F) .
\end{equation*}
\end{prop}
 
Apply 2D Fourier transform on each block diagonalizes each block $B_{i,j}$.
Defining unitary matrices $R = \frac{1}{n}(F \otimes F \otimes I_{\cout})$ and 
$Q = \frac{1}{n}(F \otimes F \otimes I_{\cin})$, change of basis can be factorized as:
\begin{equation}
\label{eq:decomposition_matrix_B}
B = R
\begin{pmatrix}
\diag(\vect{\tilde{K}_{1,1}}) & \dots & \diag(\vect{\tilde{K}_{1,\cin}}) \\
% \diag(\vect{\tilde{K}_{2,1}}) & \dots & \diag(\vect{\tilde{K}_{2,\cin}}) \\
\vdots &  & \vdots \\
\diag(\vect{\tilde{K}_{\cout, 2}}) & \dots & \diag(\vect{\tilde{K}_{\cout,\cin}})
\end{pmatrix} Q^\dag
\end{equation}

\cite{sedghi2019singular, yi2020asymptotic} propose to reshape matrix $B$ into $C$ as follows: $C = \circm{C_1, C_2, \dots, C_n}$ where $C_u = \circm{C_{u,1}, C_{u,2}, \dots, C_{u,n}}$ for $1 \leq u \leq n$, 
with $C_{u,v} = [K_{u,v,i,j}]_{i,j}$, for $1 \leq v \leq n$. 
$C$ is a doubly block circulant matrix where last level entries are $\cout \times \cin $ matrices.
%
If $B$ and $C$ represent different vectorizations of input $X$, \ie channel wise for $B$ and pixel wise for $C$ as illustrated in Figure~\ref{fig:reshape_input}, they represent the same circular convolution operator, and have the same singular values.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{graphs/reshape_input.drawio.png}
    \caption{Illustration of the vectorization performed over input $X$ depending of $B$ or $C$ matrix representation chosen for convolution operation.}
    \label{fig:reshape_input}
\end{figure}
\alexar{je comprends pas à quoi elle sert la figure 1, dans tous les cas, on ne fait jamais la vectorisation de x et la multiplcation matricelle, ce qui est important c'est lq prop 2 et 3 avec l'égalité des valeurs singulières}


\begin{prop}
\label{prop:singular_values_b_c}
\cite{henderson1981TheVM} \\
%yi2020asymptotic}
Singular values of $C$ are the same as $B$:
$\sigma(C) = \sigma(B)$ .
\end{prop} 

\cite{sedghi2019singular, yi2020asymptotic} show that applying on block level 2D Fourier transform block diagonalizes $C$.

\alexar{elle est ou la matrice C ?}

\begin{prop} 
\label{prop:blockdiagonal_cmatrix}
\cite{sedghi2019singular, yi2020asymptotic} \\
$C$ can be block diagonalized as 
\begin{equation*}
C = R
\begin{pmatrix}
G_{1,1} &  &  \\
& G_{1,2} &    \\
& & \ddots \\
&  & & G_{n,n}
\end{pmatrix} Q^\dag
\end{equation*}
with $G_{u,v} = [\tilde{K}_{i,j,u,v}]_{i,j} = [[F^\top K_{i, j} F]_{u,v}]_{i,j} \in \mathbb{C}^{\cout  \times \cin}$ for $1 \leq u,v \leq n$.
\end{prop}
\alexar{reécrire prop 2 et 3}



We use decomposition of $C$, given by Proposition \ref{prop:blockdiagonal_cmatrix}, rather than $B$ in Eq. (\ref{eq:decomposition_matrix_B}), because it is more efficient to compute singular values of a block diagonal matrix.

%Reshaping $B$ into $C$ is equivalent to reshape $\tilde{K}$ into $G$, as illustrated in Figure \ref{fig:reshape_kernel_cincout}.

%\begin{figure*}[h] \centering \includegraphics[width=1\textwidth]{graphs/reshape_kernel_cin_cout_bis_horizontal.drawio.png} \caption{Illustration of the reshape operation done over $\tilde{K} \in \mathbb{C}^{\cout \times \cin \times n \times n}$ to form $G \in \mathbb{C}^{n \times n \times \cout \times \cin}$. \\ \quentin{Attention à l'ambiguité du nom $G$}} \label{fig:reshape_kernel_cincout} \end{figure*}

Using Propositions \ref{prop:singular_values_b_c} and \ref{prop:blockdiagonal_cmatrix}, the largest singular value of a circular convolutional layer is defined as:
%\sigma_1(A) \approx 
$\sigma_1(B) = \sigma_1(C) = \max_{1 \leq u,v \leq n} \sigma_1(G_{u,v})$.
%
It remains to compute the maximum of spectral norm of all matrices $\{ G_{u,v} : 1 \leq u,v \leq n \}$.
Here this problem is convex as we consider a maximum of convex functions, as spectral norm is convex. We can note that \cite{singla2021fantastic} consider the minimum of 4 norms and thus ends up with a non convex problem.


